AuditCopilot: Leveraging LLMs for Fraud Detection in Double-Entry Bookkeeping

Auditors rely on Journal Entry Tests (JETs) to detect anomalies in tax-related ledger records, but rule-based methods generate overwhelming false positives and struggle with subtle irregularities. We investigate whether large language models (LLMs) can serve as anomaly detectors in double-entry bookkeeping. Benchmarking SoTA LLMs such as LLaMA and Gemma on both synthetic and real-world anonymized ledgers, we compare them against JETs and machine learning baselines. Our results show that LLMs consistently outperform traditional rule-based JETs and classical ML baselines, while also providing natural-language explanations that enhance interpretability. These results highlight the potential of \textbf{AI-augmented auditing}, where human auditors collaborate with foundation models to strengthen financial integrity.

==> prompt_str_4o_IF.tex <==
\begin{figure}[ht]
\centering
\begin{tikzpicture}[
  node distance=1.2cm and 1.5cm,
  box/.style={
    rectangle, draw=black, rounded corners,
    text width=6.5cm, minimum height=1cm, text centered,
    align=left, fill=gray!5, font=\small
  },
  arrow/.style={->, thick}
]

\node[box] (role) {
  \textbf{Role:} \\
  You are a financial assistant AI specialized in detecting anomalies in journal entries. Classify entries and explain findings in plain language for stakeholders.
};

\node[box, below=of role] (input) {
  \textbf{Input Format:} \\
  JSON with \texttt{posting\_id} as keys and list of transaction records. Fields include \texttt{gl\_account\_name}, \texttt{amount}, \texttt{user}, \texttt{promptly}, \texttt{weekend}, \texttt{high\_cash}, \texttt{z\_score}, etc.
};

\node[box, below=of input] (logic) {
  \textbf{Anomaly Detection Logic:} \\
  Flag anomalies if one or more apply: weekend posting, non-working hours, high-cash disbursement, top-amount, or statistical outlier. \\
  Use Isolation Forest metadata as reference — agree → high confidence; conflict → analyze \& justify.
};

\node[box, below=of logic] (output) {
  \textbf{Output Format:} \\
  JSON object per \texttt{posting\_id} with: \\
  \texttt{"Anomaly"}: 0 or 1 \\
  \texttt{"Explanation"}: 1--3 sentence rationale. \\
  \textit{Example:} \\
  \texttt{"d\_5164": \{"Anomaly": 1, "Explanation": "Posted on a weekend with high-cash disbursement. Requires review."\}}
};

% Arrows
\draw[arrow] (role.south) -- (input.north);
\draw[arrow] (input.south) -- (logic.north);
\draw[arrow] (logic.south) -- (output.north);

\end{tikzpicture}
\caption{Prompt structure used to guide GPT-4o in journal entry anomaly detection via the Hybrid Prompt. The model is conditioned through role definition, structured feature injection , interpretable logic, and a constrained output format.}
\label{fig:prompt-structure}
\end{figure}


